BENCHCOMPASS: From Scores to Signals for Training and Harness Decisions in Payment-Domain LLMs

Payment operations are a critical financial infrastructure, but the value of large language models in this domain remains unclear because payment rules change quickly, evidence is fragmented, and decisions depend on transaction state, participant role, region, and payment rail. Existing benchmarks do not isolate whether failures come from missing payment-rule knowledge, poor use of supplied evidence, or brittleness under imperfect harness inputs. We introduce BENCHCOMPASS, a payment-domain benchmark whose construction pipeline builds scenario-grounded tasks from typed evidence packs, applies LLM-based quality checks, creates task-input attack variants, and reserves final item admission for domain experts. The release contains an expert-reviewed Pro benchmark covering payment knowledge, context-grounded scenario reasoning, and Attacked Open robustness, plus a lower-assurance Normal pool for inspection and future curation. Across 16 model variants, BENCHCOMPASS shows qualitatively different failure modes: missing parametric payment knowledge, incomplete reasoning over supplied rules, and failure to reject plausible but invalid workflows. The benchmark remains unsaturated: the best frontier model reaches 89.6% on Open Context-Grounded Reasoning and 81.7% under attacked inputs, while a representative 32B open-weight model reaches 69.8% and 42.6%. Benchmark data and code are available at https://github.com/ant-intl/BenchCompass.

==> Tables/closed_open_representative_table.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Closed/Open results for representative models.} L1-C/O are L1 Closed/Open accuracies; L2-C/O are L2--L5 Closed/Open accuracies. CRR is the fraction of Closed-failed L2--L5 cases rescued by Open.}
\label{tab:closed_open_main}
\scriptsize
\setlength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabularx}{\columnwidth}{@{}P{0.24\columnwidth}P{0.16\columnwidth}ccccc@{}}
\toprule
\textbf{Model} & \textbf{Type} & \textbf{L1-C} & \textbf{L1-O} & \textbf{L2-C} & \textbf{L2-O} & \textbf{CRR} \\
\midrule
GPT-5.5 & Frontier & 77.9 & 100.0 & 36.5 & 82.3 & 75.4 \\
Gemini 3.1 Pro & Frontier & 80.0 & 100.0 & 14.6 & 89.6 & 91.5 \\
Claude Opus 4.7 & Frontier & 65.3 & 100.0 & 22.9 & 77.1 & 73.0 \\
Qwen3.5 35B & Chinese open & 58.9 & 98.9 & 17.7 & 89.6 & 88.6 \\
GLM 5.1 & Chinese closed & 65.3 & 100.0 & 15.6 & 74.0 & 72.8 \\
Gemma 4 31B & Open-weight & 56.8 & 100.0 & 5.2 & 84.4 & 83.5 \\
\bottomrule
\end{tabularx}
\end{table}


==> Tables/context_rescue_source_heatmap_figure.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.98\textwidth]{Figures/context_rescue_source_heatmap.pdf}
\caption{\textbf{Where Open context rescues representative models.} Each cell counts L2--L5 cases where a model fails Closed but passes Open, grouped by the case's primary source class. Larger counts indicate domain areas where the model lacks accessible parametric knowledge but can use the supplied source context.}
\label{fig:app_context_rescue_heatmap}
\end{figure*}


==> Tables/qwen_model_scaling_figure.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.88\textwidth]{Figures/qwen_model_scaling.pdf}
\caption{\textbf{Model scaling behaves differently across diagnostic subsets.} The Qwen3 panel uses explicit non-thinking runs; the Qwen3.5 panel uses Bailian default-thinking runs.}
\label{fig:qwen_model_scaling}
\end{figure*}


==> Tables/representative_open_failure_mode_table.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Manual audit of representative Open failures.} Counts are model--case errors for six representative models on L2--L5 Open cases. The audit separates substantive context-use errors from residual judge/rubric sensitivity.}
\label{tab:app_open_failure_modes}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\textwidth}{@{}P{0.22\textwidth}ccP{0.31\textwidth}Y@{}}
\toprule
\textbf{Failure mode} & \textbf{Model-case} & \textbf{Cases} & \textbf{What failed} & \textbf{Typical cases} \\
\midrule
Multi-rule synthesis & 26 & 12 & Retrieves local facts but fails to combine rules, precedence, workflow order, or causal relations. & CPMI stability, CHAPS/CLS fallback, SVF onboarding \\
Scope or exception boundary & 26 & 10 & Misapplies an exclusion, exception, entity role, jurisdictional scope, or transaction-state boundary. & CHATS member exclusion, all-or-none, reporting boundary \\
Over-expanded answer path & 18 & 7 & Adds extra rules, exceptions, or operational actions that change or obscure the requested decision. & Visa OCT, Buna access, PayPal refund \\
Modal or threshold precision & 17 & 10 & Confuses may/must, possible/certain, immediate/conditional, or a numeric/date threshold. & Zelle possible delay, ISO 20022 may need, 21-day conversion \\
Judge/rubric sensitivity & 7 & 5 & The answer is substantially correct, but automatic scoring is sensitive to extra wording or missing exact phrasing. & offshore RMB conversion, same-day bill payment \\
Liability or responsibility boundary & 5 & 3 & Does not cleanly assign responsibility among platforms, banks, providers, or users. & Western Union wallet, BOCHK e-CNY, gateway vs escrow \\
\bottomrule
\end{tabularx}
\end{table*}


==> Tables/source_role_bubble_heatmap_figure.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.86\textwidth]{Figures/source_role_bubble_heatmap.pdf}
\caption{\textbf{Coverage across benchmark subsets, dot-matrix view.} Bubble area encodes case count for each coverage class and benchmark subset. This optional view reduces the visual dominance of high-count infrastructure categories.}
\label{fig:source_role_bubble_heatmap}
\end{figure*}


==> Tables/source_role_distribution_figure.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{Figures/source_distribution_old_taxonomy.pdf}
\caption{\textbf{Payment-domain coverage of the final release.} Each case is counted once by its primary evidence class. Bars are sorted by total count and split by benchmark subset. The taxonomy separates payment-system access, payment-message standards, currency exchange, remittance, regulators, banks, payment platforms, card networks, clearing and settlement, and digital wallets.}
\label{fig:source_role_distribution}
\end{figure}

